8-13 micron spectroscopy of NGC 253: a spatially resolved starburst

NGC 253 is a nearby spiral galaxy that is currently undergoing a nuclear burst of star formation in a 100 pc diameter region. We present spatially resolved 8--13 micron low-resolution spectra at four positions along the ridge of 8--13 micron emission. We find that the relative strengths of the ionic, dust emission features, and dust continuum emission vary with position in the galaxy but can be accounted for everywhere without recourse to extinction by silicates. The brightest mid-infrared peak (which is displaced from the nucleus) has elevated levels of both continuum and 11.1--12.9 micron `plateau' emission, indicative of dust heated within a photo-dissociation region. Spectra obtained over the course of 3 yr at the position of the brightest mid-infrared peak show no significant time variation.

==> mntable.tex <==
\def\tablenotemark#1{\rlap{$^{\rm #1}$}}
\newtoks\@temptokenb
\def\tblnote@list{}
\def\tablenotetext#1#2{
\@temptokena={\vspace{.5ex}{\noindent\llap{$^{#1}$}#2}\par}
\@temptokenb=\expandafter{\tblnote@list}
\xdef\tblnote@list{\the\@temptokenb\the\@temptokena}}
\def\spew@tblnotes{
\ifx\tblnote@list\@empty\relax
\else
\vspace{4.5ex}
\footnoterule
\vspace{.5ex}
{\footnotesize\tblnote@list}
\gdef\tblnote@list{}
\fi}
\def\endtable{\spew@tblnotes\end@float}
\@namedef{endtable*}{\spew@tblnotes\end@dblfloat}
\let\tableline=\hline
\long\def\@makecaption#1#2{\vskip 2ex\noindent #1 #2\par}
\def\tablenum#1{\def\thetable{#1}\let\@currentlabel\thetable
\addtocounter{table}{\m@ne}}
\def\figurenum#1{\def\thefigure{#1}\let\@currentlabel\thefigure
\addtocounter{figure}{\m@ne}}
\let\placetable=\@gobble
\let\placefigure=\@gobble
\let\placeplate=\@gobble
\def\figcaption{\@ifnextchar[{\@xfigcaption}{\@figcaption}}
\def\@figcaption#1{{\def\@captype{figure}\caption{#1}}}
\def\@xfigcaption[#1]#2{{\def\@captype{figure}\caption{#2}}}
\def\dummytable{\refstepcounter{table}}
\newbox\pt@box
\newdimen\pt@width
\newcount\pt@line
\newcount\pt@column
\newcount\pt@nlines
\newcount\pt@ncol
\newcount\pt@page
\newdimen\mnlinewidth
\let\mnlinewidth\columnwidth
\newdimen\mnptwidth

\let\@mnfloat=\@dblfloat
\let\end@mnfloat=\end@dblfloat

%\ifdim\mnptwidth>\mnlinewidth\let\@mnfloat=\@dblfloat\else\let\@mnfloat=\@float\fi
%\ifdim\mnptwidth>\mnlinewidth\let\end@mnfloat=\end@dblfloat\else\let\end@mnfloat=\end@float\fi


\def\colhead#1{\multicolumn{1}{c}{#1}\pt@addcol}
\def\tablecolumns#1{\pt@column=#1\pt@ncol=#1\gdef\pt@addcol{\relax}}
\def\tablecaption#1{\gdef\pt@caption{#1}} \def\pt@caption{\relax}
\def\tablehead#1{\gdef\pt@head{\hline\relax\\[-1.7ex]
#1\hskip\tabcolsep\\[.7ex]\hline\relax\\[-1.5ex]}} \def\pt@head{\relax}
\def\tabletail#1{\gdef\pt@tail{#1}} \def\pt@tail{\relax}
\def\tablewidth#1{\pt@width=#1} \pt@width\textwidth
\def\tableheadfrac#1{\gdef\pt@headfrac{#1}} \def\pt@headfrac{.1}
\def\pt@calcnlines{\@tempdima\pt@headfrac\textheight
\@tempdimb\textheight\advance\@tempdimb by-\@tempdima
\@tempdima\arraystretch\baselineskip
\divide\@tempdimb by\@tempdima
\global\pt@nlines\@tempdimb}
\def\pt@tabular{\hbox \bgroup $\let\@acol\@ptabacol
\let\@classz\@tabclassz
\let\@classiv\@tabclassiv \let\\\@tabularcr\@tabarray}
\def\@ptabacol{\edef\@preamble{\@preamble \hskip \tabcolsep\tabskip\fill}}
\def\fnum@ptable{Table \thetable}
\def\fnum@ptablecont{Table \thetable---{\rm Continued}}
\newdimen\pt@tmpcapwidth
\def\set@mkcaption{\long\def\@makecaption##1##2{\ifdim\pt@width>\z@%
\pt@tmpcapwidth\pt@width\else\pt@tmpcapwidth\textwidth\fi%
\parbox{\pt@tmpcapwidth}{\rm##1.\quad##2}%
}}
\def\set@mkcaptioncont{\long\def\@makecaption##1##2{
\rm##1\vskip 2.5ex}}
\newenvironment{deluxetable}[1]{\def\pt@format{\string#1}%
\set@tblnotetext\global\pt@ncol=0\global\pt@column=0\global\pt@page=1%
\def\pt@addcol{\global\advance\pt@ncol by\@ne}}%
{\mnptwidth\wd\pt@box%
\pt@width\wd\pt@box\box\pt@box\spew@ptblnotes%
\typeout{Page \the\pt@page\space of table \thetable\space has been set to
width \the\pt@width\space with \the\pt@nlines\space lines per page. The columnwidth is \the\mnlinewidth .  The table width is \the\mnptwidth . }%
%\let\mnptwidth\pt@width%
\end@mnfloat}
\let\planotable=\deluxetable
\let\endplanotable=\enddeluxetable
\def\startdata{\pt@line=0\pt@calcnlines%
\ifdim\pt@width>\z@\def\@halignto{to \pt@width}\else\def\@halignto{}\fi%
\mnptwidth\wd\pt@box\typeout{\the\mnptwidth}
\let\fnum@table=\fnum@ptable\set@mkcaption%
\@mnfloat{table}\caption{\pt@caption}\leavevmode%
\setbox\pt@box=\pt@tabular{\pt@format}\pt@head}
\def\enddata{\crcr\noalign{\vskip .7ex}\hline\endtabular}
\def\pt@nl{\global\advance\pt@line by\@ne%
\ifnum\pt@line=\pt@nlines%
\endtabular\pt@width\wd\pt@box\box\pt@box
\typeout{Page \the\pt@page\space of table \thetable\space has been set to
width \the\pt@width}%
\global\advance\pt@page by\@ne%
\end@mnfloat\clearpage%
\addtocounter{table}{\m@ne}%
\let\fnum@table=\fnum@ptablecont\set@mkcaptioncont%
\@mnfloat{table}\caption[\null]{\pt@caption}\leavevmode%
\global\pt@ncol=\pt@column
\global\pt@line=0%
\setbox\pt@box=\pt@tabular{\pt@format}\pt@head%
\else\\
\fi}
\let\nl=\pt@nl
\let\nextline=\pt@nl
\def\tablevspace#1{\noalign{\vskip#1}}
\def\tablebreak{\pt@line\pt@nlines\advance\pt@line by\m@ne\pt@nl}
\def\cutinhead#1{\noalign{\vskip 1.5ex}
\hline\pt@nl\noalign{\vskip -2.0ex}
\multicolumn{\pt@ncol}{c}{#1}\pt@nl
\noalign{\vskip .8ex}
\hline\pt@nl\noalign{\vskip -2ex}}
\def\sidehead#1{\noalign{\vskip 1.5ex}
\multicolumn{\pt@ncol}{@{\hskip\z@}l}{#1}\pt@nl
\noalign{\vskip .5ex}}
\def\set@tblnotetext{\def\tablenotetext##1##2{{%
\@temptokena={{\parbox{\pt@width}{\hskip1em$^{\rm ##1}$##2}}\par}%
\@temptokenb=\expandafter{\tblnote@list}
\xdef\tblnote@list{\the\@temptokenb\the\@temptokena}}}}
\def\spew@ptblnotes{
\ifx\tblnote@list\@empty\relax
\else
\par
\vspace{2ex}
{\parskip=1.5ex%
\tblnote@list}
\gdef\tblnote@list{}
\fi}
\def\tablerefs#1{\@temptokena={\vspace*{3ex}{%
\parbox{\pt@width}{\hskip1em\rm References. --- #1}\par}}%
\@temptokenb=\expandafter{\tblnote@list}
\xdef\tblnote@list{\the\@temptokenb\the\@temptokena}}
\def\tablecomments#1{\@temptokena={\vspace*{3ex}{%
\parbox{\pt@width}{\hskip1em\rm Note. --- #1}\par}}%
\@temptokenb=\expandafter{\tblnote@list}
\xdef\tblnote@list{\the\@temptokenb\the\@temptokena}}
\def\thetable{\@arabic\c@table}
\def\fnum@table{{\rm Table \thetable:}}
\def\fps@table{h}
\def\phn{\phantom{0}}
\def\phd{\phantom{.}}
\def\phs{\phantom{$-$}}
\def\nodata{ ~$\cdots$~ }

